Affective Computing Has Changed: The Foundation Model Disruption

The dawn of Foundation Models has on the one hand revolutionised a wide range of research problems, and, on the other hand, democratised the access and use of AI-based tools by the general public. We even observe an incursion of these models into disciplines related to human psychology, such as the Affective Computing domain, suggesting their affective, emerging capabilities. In this work, we aim to raise awareness of the power of Foundation Models in the field of Affective Computing by synthetically generating and analysing multimodal affective data, focusing on vision, linguistics, and speech (acoustics). We also discuss some fundamental problems, such as ethical issues and regulatory aspects, related to the use of Foundation Models in this research area.

==> tables/audio_va_prompt.tex <==
\begin{table}[ht!]
    \centering
    \caption{Prompt templates for valence/arousal prediction from speech with LLaMa\,2 based on eGeMAPS features. The slash indicates an alternative, i.\,e., the valence-related parts are used to create the valence prompt only, and, analogously, the arousal-related parts are only used to construct the arousal prompt.}
    \label{tab:va_speech_prompt}
    \begin{tabular}{l}
    \toprule
    \textbf{Prompt template}\\
    \midrule
    Suppose you are given the following eGeMAPS feature values for a speech sample: \\ 
    F0semitioneFrom27.5Hz\_sma3nz\_amean: 24.66\\
    ... \\
    Given these values, please estimate the degree of \emph{arousal, i.\,e., activation}/\emph{valence, i.\,e., pleasantness},\\ exhibited in this sample. Answer with an integer value between 0 and 100. \emph{Arousal}/\emph{Valence} value: \\
    
    %\texttt{[text]}\\ 
    %\#Output phrase:\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/text_analysis_prompts.tex <==
% \begin{table}[ht!]
%     \centering
%     \caption{Prompt template for transforming neutral sentences into emotionally charged versions using foundation models.}
%     \label{tab:emotion_transformation_template}
%     \begin{tabular}{l}
%     \toprule
%     \textbf{Prompt template}\\
%     \midrule
%     \#Instruction:You are an expert in affective computing and psychology. Your task is to \\ transform a neutral sentence into an emotionally charged version without using emojis,\\ symbols, or any forms of non-verbal expression. When  presented with the neutral phrase,\\ convert it into a sentence with a  strong and intense sense of \texttt{[emotion]} emotion while adapting\\ it into a formal style of language and not explaining or adding anything in addition.\\[0.2cm]   \#Rules:\\
%     - Avoid explanations, titles, and irrelevant characters like emojis, etc. \\ - Ensure that all original facts are preserved.\\[0.2cm] 
%     \#Neutral phrase:
%     \texttt{[text]}\\ 
%     \#Output phrase:\\
%     \bottomrule
%     \end{tabular}
% \end{table}
\begin{table}[ht!]
    \centering
    \caption{Prompt template for classifying dominant emotions in given text using foundation models.}
    \label{tab:emotion_classification_template}
    \begin{tabular}{l}
    \toprule
    \textbf{Prompt template}\\
    \midrule
    You are an expert in affective computing. Given a text by the user, \\ analyse which emotion is most dominant in the given text. Only \\classify one of the seven Ekman emotions, namely: `anger`, `disgust`,\\ `fear`, `joy`, `neutral`, `sadness`, `surprise`. \\...\\Just write the emotion, and nothing else.\\[0.2cm] 
    \bottomrule
    \end{tabular}
\end{table}

==> tables/text_generation_prompts.tex <==
% \begin{table}[ht!]
%     \centering
%     \caption{Prompt template for transforming neutral sentences into emotionally charged versions using foundation models.}
%     \label{tab:emotion_transformation_template}
%     \begin{tabular}{l}
%     \toprule
%     \textbf{Prompt template}\\
%     \midrule
%     \#Instruction:You are an expert in affective computing and psychology. Your task is to \\ transform a neutral sentence into an emotionally charged version without using emojis,\\ symbols, or any forms of non-verbal expression. When  presented with the neutral phrase,\\ convert it into a sentence with a  strong and intense sense of \texttt{[emotion]} emotion while adapting\\ it into a formal style of language and not explaining or adding anything in addition.\\[0.2cm]   \#Rules:\\
%     - Avoid explanations, titles, and irrelevant characters like emojis, etc. \\ - Ensure that all original facts are preserved.\\[0.2cm] 
%     \#Neutral phrase:
%     \texttt{[text]}\\ 
%     \#Output phrase:\\
%     \bottomrule
%     \end{tabular}
% \end{table}
% \begin{table}[!t]
%     \centering
%     \begin{tabular}{l}
%     \toprule
%     \textbf{Prompt template}\\
%     \midrule
%     You are an expert in affective computing. Given a text by the user, \\ analyse which emotion is most dominant in the given text. Only \\classify one of the seven Ekman emotions, namely: `anger`, `disgust`,\\ `fear`, `joy`, `neutral`, `sadness`, `surprise`. \\...\\Just write the emotion, and nothing else.\\[0.2cm] 
%     \bottomrule
%     \end{tabular}
%     \caption{Prompt template for classifying dominant emotions in given text using foundation models.}
%     \label{tab:emotion_classification_template}
% \end{table}
